Resummation for Nonequilibrium Perturbation Theory and Application to Open Quantum Lattices

Lattice models of fermions, bosons, and spins have long served to elucidate the essential physics of quantum phase transitions in a variety of systems. Generalizing such models to incorporate driving and dissipation has opened new vistas to investigate nonequilibrium phenomena and dissipative phase transitions in interacting many-body systems. We present a framework for the treatment of such open quantum lattices based on a resummation scheme for the Lindblad perturbation series. Employing a convenient diagrammatic representation, we utilize this method to obtain relevant observables for the open Jaynes-Cummings lattice, a model of special interest for open-system quantum simulation. We demonstrate that the resummation framework allows us to reliably predict observables for both finite and infinite Jaynes-Cummings lattices with different lattice geometries. The resummation of the Lindblad perturbation series can thus serve as a valuable tool in validating open quantum simulators, such as circuit-QED lattices, currently being investigated experimentally.

==> arXiv submission/header_command.tex <==
%\newcounter{fig}
%\newenvironment{romenu}{\begin{list}{(\roman{fig})}{\usecounter{fig} %\setlength{\labelwidth}{1.5cm}}}{\end{list}}
%\newenvironment{arabenu}{\begin{list}{(\arabic{fig})}{\usecounter{fig} %\setlength{\labelwidth}{1.5cm}}}{\end{list}}


\renewcommand{\rho}{\text{\textrho}}
\renewcommand{\sigma}{\text{\textsigma}}
\newcommand{\oket}[1]{\left|#1\right)}
\newcommand{\oketb}[1]{\Big|#1\Big)}
\newcommand{\oketn}[1]{|#1)}
\newcommand{\omat}[3]{\left( #1 \right| #2 \left| #3 \right)}
\newcommand{\omatb}[3]{\Big( #1 \Big| #2 \Big| #3 \Big)}
\newcommand{\omatn}[3]{( #1 | #2 | #3 )}



%Command
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\nn}{\nonumber}
\newcommand{\lf}{\left}
\newcommand{\rt}{\right}

%Quick symbol
\DeclareMathOperator{\Tr}{tr}
%\newcommand{\mo}{\mathcal{O}}

\newcommand{\dg}{^{\da}}
\newcommand{\ddg}{^{\dda}}
\newcommand{\da}{\dagger}
\newcommand{\dda}{\da \hspace{-2pt} \da}
\newcommand{\pinv}{^{\leftharpoonup 1}}
\newcommand{\ginv}{^{-1}}

\newcommand{\alp}{\alpha}
\newcommand{\ep}{\epsilon}
\newcommand{\ld}{\lambda}
\newcommand{\s}{\sigma}
%\newcommand{\ze}{\zeta}

\newcommand{\dw}{\delta \omega}
\newcommand{\dwr}{\dw}
\newcommand{\dwrm}[1]{\dw_{#1}}
\newcommand{\dwrk}{\dwrm{\vk}}
\newcommand{\dwq}{\delta \Omega}

\newcommand{\ga}{\gamma}
\newcommand{\gar}{\ga}
\newcommand{\gaq}{\Gamma}

\newcommand{\epe}{\ep_{\mathrm{q}}}

\newcommand{\alpt}{\tilde{\alp}}
\newcommand{\at}{\tilde{\mathsf{a}}}
\newcommand{\bt}{\mathsf{b}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\am}{\at_{\vm}}

\newcommand{\vm}{\mathbf{0}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vp}{\mathbf{r}}

\newcommand{\ka}{\kappa}
\newcommand{\kadi}{\ka_{\textrm{di}}}
\newcommand{\kach}{\ka_{\textrm{ch}}}
\newcommand{\kagl}{\ka_{\textrm{gl}}}

%Function
\newcommand{\vpi}[1]{\vp_{\mathbf{#1}}}
\newcommand{\vki}[1]{\vk_{\mathbf{#1}}}

\newcommand{\abs}[1]{\lf| #1 \rt|} 
%\newcommand{\Reb}[1]{\mathrm{Re} \lf[ #1 \rt]}
%\newcommand{\sReb}[1]{\mathrm{Re} [ #1 ]}
%\newcommand{\Imb}[1]{\mathrm{Im} \lf[ #1 \rt]}
%\newcommand{\sImb}[1]{\mathrm{Im} [ #1 ]}
\newcommand{\Trb}[1]{\mathrm{tr} \lf[ #1 \rt]}
\newcommand{\sTrb}[1]{\mathrm{tr} [ #1 ]}

\newcommand{\avg}[1]{\left< #1 \right>}
\newcommand{\savg}[1]{\langle #1 \rangle}

\newcommand{\expap}[2]{\avg{#1}^{\lf(#2\rt)}}
\newcommand{\sexpap}[2]{\savg{#1}^{\lf(#2\rt)}}



\newcommand{\inner}[2]{\left(#1|#2\right)}
\newcommand{\sinner}[2]{( #1|#2 )}




\newcommand{\sPf}[4]{\sP^{#1#2}_{#3#4}}

\newcommand{\sCom}[1]{\lf[#1 , {}_\bullet \rt]}

%Spin
\newcommand{\si}[2]{\s^{#1}_{#2}}
\newcommand{\spl}[1]{\si{+}{#1}}
\newcommand{\smi}[1]{\si{-}{#1}}

\newcommand{\spvp}{\spl{\vp}}
\newcommand{\smvp}{\smi{\vp}}

%Third-quantization super-operator
\newcommand{\sNmaev}[1]{t_{#1}}
\newcommand{\sNmbev}[1]{\tau_{#1}}

\newcommand{\sNma}[1]{\srr{#1}}
\newcommand{\sNmb}[1]{\sbb{#1}}
\newcommand{\sNmap}[1]{\sbap{#1}}
\newcommand{\sNmbp}[1]{\sbbp{#1}}

%Third-quantization super-operator
\newcommand{\sbasym}{\mathbb{b}}
\newcommand{\sbbsym}{\bbbeta}
\newcommand{\sba}[1]{\sbasym_{#1}}
\newcommand{\sbb}[1]{\sbbsym_{#1}}
\newcommand{\sbap}[1]{\sbasym^{\dda}_{#1}}
\newcommand{\sbbp}[1]{\sbbsym^{\dda}_{#1}}

\newcommand{\sbavk}{\sba{\vk}}
\newcommand{\sbbvk}{\sbb{\vk}}
\newcommand{\sbapvk}{\sbap{\vk}}
\newcommand{\sbbpvk}{\sbbp{\vk}}

\newcommand{\ssl}[2]{\mathbb{s}^{#1}_{#2}}
\newcommand{\ssr}[2]{\bbsigma^{#1}_{#2}}
\newcommand{\ssml}[1]{\ssl{-}{#1}}
\newcommand{\sspl}[1]{\ssl{+}{#1}}
\newcommand{\ssmr}[1]{\ssr{-}{#1}}
\newcommand{\sspr}[1]{\ssr{+}{#1}}

\newcommand{\ssmlvp}{\ssml{\vp}}
\newcommand{\ssplvp}{\sspl{\vp}}
\newcommand{\ssmrvp}{\ssmr{\vp}}
\newcommand{\ssprvp}{\sspr{\vp}}

%Liouvillian
\newcommand{\sL}{\mathbb{L}}
\newcommand{\sLr}[1]{\sL_{r}^{#1}}
\newcommand{\sLq}[1]{\sL_{q}^{#1}}
\newcommand{\sLrq}[2]{\sL_{rq}^{#1 #2}}

%Super-operator
\newcommand{\sA}{\mathbb{A}}
\newcommand{\sD}{\mathbb{D}}

\newcommand{\spf}[1]{\mathbb{f}_{#1}}
\newcommand{\spSE}[1]{\bbsigma_{#1}}

\newcommand{\sU}{\mathbb{U}}
%\newcommand{\sUp}{\sU'}
\newcommand{\sUp}{\mathbb{T}}
\newcommand{\sUpc}[1]{\sUp_{#1}}

\newcommand{\sUkp}[2]{\sU^{#1 #2}}
\newcommand{\sUpckp}[3]{\sU_{#1}^{\prime #2 #3}}

%\newcommand{\sBa}[2]{\mathbb{V}_{#1 #2}}
%\newcommand{\sBap}[2]{\mathbb{V}^{\dda}_{#1 #2}}
%\newcommand{\sBb}[2]{\mathbb{W}_{#1 #2}}
%\newcommand{\sBbp}[2]{\mathbb{W}^{\dda}_{#1 #2}}
%\newcommand{\sBavk}[1]{\sBa{\vk}{#1}}
%\newcommand{\sBapvk}[1]{\sBap{\vk}{#1}}
%\newcommand{\sBbvk}[1]{\sBb{\vk}{#1}}
%\newcommand{\sBbpvk}[1]{\sBbp{\vk}{#1}}
%\newcommand{\sBavkvp}{\sBa{\vk}{\vp}}
%\newcommand{\sBapvkvp}{\sBap{\vk}{\vp}}
%\newcommand{\sBbvkvp}{\sBb{\vk}{\vp}}
%\newcommand{\sBbpvkvp}{\sBbp{\vk}{\vp}}

%Loop correction
\newcommand{\selfe}{\mathbb{\SavedSigma}}
\newcommand{\sloop}{\mathbb{\SavedSigma}}
\newcommand{\ssloop}{\tilde{\sloop}}
\newcommand{\sloopn}[1]{\sloop_{#1}}
\newcommand{\evasloop}{\Sigma}
\newcommand{\evassloop}{\tilde{\Sigma}}
\newcommand{\evasloopn}[3]{\evasloop_{#1;#3}^{#2}}


%Liouville super-operator eigenstates
\newcommand{\evr}[1]{\mathsf{u}_{#1}}
\newcommand{\evl}[1]{\breve{\mathsf{u}}_{#1}}
\newcommand{\eva}[1]{\mathsf{\ld}_{#1}}

\newcommand{\evrc}[2]{\mathsf{u}_{#1}^{#2}}
\newcommand{\evlc}[2]{\breve{\mathsf{u}}_{#1}^{#2}}
\newcommand{\evac}[2]{\ld_{#1}^{#2}}

%Resonator eigenstates
\newcommand{\evrr}[3]{\mathsf{r}^{#1}_{#2#3}}
\newcommand{\evlr}[3]{\breve{\mathsf{r}}^{#1}_{#2#3}}
\newcommand{\evar}[3]{\mathsf{\ld}^{#1}_{#2#3}}
\newcommand{\evrrvk}[2]{\evrr{\vk}{#1}{#2}}
\newcommand{\evarvk}[2]{\evar{\vk}{#1}{#2}}
\newcommand{\evlrvk}[2]{\evlr{\vk}{#1}{#2}}
\newcommand{\evrs}[1]{\evrr{#1}{0}{0}}
\newcommand{\evrsvk}{\evrrvk{0}{0}}

%Qubit eigenstates
\newcommand{\evrq}[2]{\mathsf{q}^{#1}_{#2}}
\newcommand{\evlq}[2]{\breve{\mathsf{q}}^{#1}_{#2}}
\newcommand{\evaq}[2]{\ell^{#1}_{#2}}
\newcommand{\evrqvp}[1]{\evrq{\vp}{#1}}
\newcommand{\evlqvp}[1]{\evlq{\vp}{#1}}
\newcommand{\evaqvp}[1]{\evaq{\vp}{#1}}
\newcommand{\evqs}[1]{\evrq{#1}{0}}
\newcommand{\evqsvp}{\evrqvp{0}}

%Density matrix
\newcommand{\rs}{\rho_\mathrm{s}}
\newcommand{\rsc}[1]{\rho^{[ #1]}}
\newcommand{\rscp}[2]{\rho_{#2}^{[ #1]}}
\newcommand{\rscl}[1]{\breve{\rho}^{[ #1]}}
\newcommand{\rscpl}[2]{\breve{\rho}_{#2}^{[ #1]}}

\newcommand{\rso}{\rho_{\mathrm{s}}}
\newcommand{\rsoc}[1]{\rho_{ #1}}

%\newcommand{\nullone}[2]{\rscp{0}{\cancel{#1} \cancel{#2}}}
%\newcommand{\rhotwo}[2]{\rho^{#1}_{#2}}


\newcommand{\msar}{\mathsf{a}_{\vp}}
\newcommand{\msbk}{\mathsf{b}_{\vk}}



==> arXiv submission/header_preserve.tex <==
\let\SavedLambda\Lambda
\let\SavedSigma\Sigma
